SimpleTrack: Understanding and Rethinking 3D Multi-object Tracking

3D multi-object tracking (MOT) has witnessed numerous novel benchmarks and approaches in recent years, especially those under the "tracking-by-detection" paradigm. Despite their progress and usefulness, an in-depth analysis of their strengths and weaknesses is not yet available. In this paper, we summarize current 3D MOT methods into a unified framework by decomposing them into four constituent parts: pre-processing of detection, association, motion model, and life cycle management. We then ascribe the failure cases of existing algorithms to each component and investigate them in detail. Based on the analyses, we propose corresponding improvements which lead to a strong yet simple baseline: SimpleTrack. Comprehensive experimental results on Waymo Open Dataset and nuScenes demonstrate that our final method could achieve new state-of-the-art results with minor modifications. Furthermore, we take additional steps and rethink whether current benchmarks authentically reflect the ability of algorithms for real-world challenges. We delve into the details of existing benchmarks and find some intriguing facts. Finally, we analyze the distribution and causes of remaining failures in \name\ and propose future directions for 3D MOT. Our code is available at https://github.com/TuSimple/SimpleTrack.

==> 4-setup.tex <==
\section{Validation Set Up}
\label{sec::setup}
(This section may go to supplementary if not enough place.)
As demonstrated in Fig~\ref{fig::progress}, our analyses and improvements start from the common baselines of AB3DMOT~\cite{ab3dmot} and Chiu \etal~\cite{mdis}. Due to the different settings and metrics on Waymo Open Dataset and NuScenes Dataset, we adapt the algorithms, including their strategies and hyper-parameters, on each benchmark regarding the final performance. In this section, we describe the baseline of our implementations, which are followed by our gradual improvements in Sec.~\ref{sec::ablation}.

For Waymo Open Dataset:
\begin{itemize}[itemsep=-1mm]
    \item \textit{Initialization Model}. We use center point detection~\cite{center_point}, and filter detection bounding boxes with 0.7 for vehicles and cyclists, and 0.5 for pedestrians.
    \item \textit{Association}. For AB3DMOT~\cite{ab3dmot}, we keep the IOU function and Hungarian algorithm for association, and use $\texttt{IOU}_{\texttt{3D}}>0.1$ as the threshold for successful association. For Chiu \etal~\cite{mdis}, we use Mahalanobis distance, greedy algorithm, and the distance threshold of 5 as successful association.
    \item \textit{Motion Model}. We use the default Kalman filter parameters as AB3DMOT~\cite{ab3dmot}, and re-estimate the parameters for Chiu \etal~\cite{mdis} with the same algorithm.
    \item \textit{Life Cycle Management}. The life cycle management is the same as AB3DMOT~\cite{ab3dmot}.
\end{itemize}

For NuScenes:
\begin{itemize}[itemsep=-1mm]
    \item \textit{Initialization Model}. For the AMOTA evaluation metrics, we keep all the output from the center point~\cite{center_point} detections.
    \item \textit{Association}. For AB3DMOT~\cite{ab3dmot}, we use the same approach as on the Waymo Open Dataset mentioned above. For Chiu \etal~\cite{mdis}, we rigorously follow the setting in their original paper.
    \item \textit{Motion Model}. Same as on the Waymo Open Dataset, we use the default parameters for AB3DMOT~\cite{ab3dmot}, and re-estimate the parameters \textit{w.r.t} the center point detection for Chiu \etal~\cite{mdis}.
    \item \textit{Life Cycle Management}. We adopt the same strategy as the tracking algorithm in center point~\cite{center_point}, where the trackers start outputting on the first association.
\end{itemize}
